Exploring the Potential of Synthetic Data to Replace Real Data

The potential of synthetic data to replace real data creates a huge demand for synthetic data in data-hungry AI. This potential is even greater when synthetic data is used for training along with a small number of real images from domains other than the test domain. We find that this potential varies depending on (i) the number of cross-domain real images and (ii) the test set on which the trained model is evaluated. We introduce two new metrics, the train2test distance and $\text{AP}_\text{t2t}$, to evaluate the ability of a cross-domain training set using synthetic data to represent the characteristics of test instances in relation to training performance. Using these metrics, we delve deeper into the factors that influence the potential of synthetic data and uncover some interesting dynamics about how synthetic data impacts training performance. We hope these discoveries will encourage more widespread use of synthetic data.

==> Contents/preamble.tex <==
\usepackage{caption}
\usepackage{subcaption}
\usepackage{times}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{url}
\usepackage{xcolor}
\usepackage{Styles/spconf}
% Title.
% ------
\title{Exploring the potential of synthetic data to replace real data}
%
% Single address.
% ---------------
%\name{Author(s) Name(s)\thanks{Thanks to XYZ agency for funding.}}
%\name{Author(s)}
%\address{Author Affiliation(s)}
%\name{Yan Zhang$^{\star,1}$~~~~~~~~~~Hyungtae Lee$^{\star,2}$~~~~~~~~~~Heesung Kwon$^{2}$~~~~~~~~~~Shuvra S. Bhattacharyya$^{1}$ \vspace{-0.8em}}
%\address{$^{\star}$ {\normalsize equal contribution}\vspace{0.5em}\\$^{1}$ University of Maryland, College Park~~~~~~~~~~$^{2}$ DEVCOM Army Research Laboratory}
\name{Hyungtae Lee$^{\star,1}$~~~~~~~~~~Yan Zhang$^{\star,2}$~~~~~~~~~~Heesung Kwon$^{3}$~~~~~~~~~~Shuvra S. Bhattacharyya$^{2}$ \vspace{-0.8em}}
\address{$^{\star}$ {\normalsize equal contribution}\vspace{0.5em}\\$^{1}$ BlueHalo~~~~~$^{2}$ University of Maryland, College Park~~~~~$^{3}$ DEVCOM Army Research Laboratory}
%\date{June 2023}

%
% For example:
% ------------
%\address{School\\
%	Department\\
%	Address}
%
% Two addresses (uncomment and modify for two-address case).
% ----------------------------------------------------------
%\twoauthors
%  {A. Author-one, B. Author-two\sthanks{Thanks to XYZ agency for funding.}}
%	{School A-B\\
%	Department A-B\\
%	Address A-B}
%  {C. Author-three, D. Author-four\sthanks{The fourth author performed the work
%	while at ...}}
%	{School C-D\\
%	Department C-D\\
%	Address C-D}



